Neural Random-Access Machines

In this paper, we propose and investigate a new neural network architecture called Neural Random Access Machine. It can manipulate and dereference pointers to an external variable-size random-access memory. The model is trained from pure input-output examples using backpropagation. We evaluate the new model on a number of simple algorithmic tasks whose solutions require pointer manipulation and dereferencing. Our results show that the proposed model can learn to solve algorithmic tasks of such type and is capable of operating on simple data structures like linked-lists and binary trees. For easier tasks, the learned solutions generalize to sequences of arbitrary length. Moreover, memory access during inference can be done in a constant time under some assumptions.

==> hyperparameters.tex <==
\section{Hyperparameters}\label{app:hyper}

In this section we provide detailed information about the hyperparameters we use, which should allow to replicate our results.
In Sec.~\ref{app:desc} we describe all the hyperparameters we use.
Some of the hyperparameters were fixed across all experiments, e.g. we always trained the model for $100$ epochs.
The values of such hyperparameters are listed in Sec.~\ref{app:desc}.

The remaining hyperparameters were drawn using random sampling.
In Sec.~\ref{app:values} we list the best values of the hyperparameters we found for each problem.




\subsection{Description of the hyperparameters}\label{app:desc}

The following settings were fixed for all the experiments we've done:
\begin{enumerate}
 \item We trained the model for $100$ epochs, each consisting of $1000$ batches.
 \item We used batch size $100$ (or $50$ if we exceeded GPU memory).
 \item After each epoch we measured the error on $100$ batches with the model parameters fixed.
 \item The memory size was equal $32$ during training.
 To test generalization of the model to longer input sequences we used the smallest memory size allowing to store input and output leaving at least $2$ empty memory cells.
 \item We used $\epsilon=10^{-30}$ to clip the values of logarithms. See paragraph ,,Limiting the values of logarithms'' in Sec.~\ref{sec:train} for more information.
 %\item max_output_prob 0.8
\end{enumerate}

The following hyperparameters were drawn suing random smapling:
\begin{enumerate}
 \item \textbf{init\_h}: the initial values of the parameters are sampled uniformly from the range $(-\mathbf{init\_h},\mathbf{init\_h})$.
 \item \textbf{learning\_rate}: notice that the cost function we use is a \emph{sum} of the negative log-likelihoods of all output memory cells in the whole batch.
 \item \textbf{lr\_decay}: learning rate is multiplied by this value after every epoch.
 \item \textbf{adam\_eps}: $\epsilon$ parameter for the Adam optimization algorithm.
 The remaining parameters of the Adam algorithm were set exactly as in the original paper \cite{kingma2014adam}.
 \item \textbf{max\_grad\_norm}: gradient is scaled down if its L2 norm exceeds this value.
 \item \textbf{grad\_crop}: the maximum allowed L1 norm of gradients w.r.t. intermediate values (higher values are cropped).
 \item \textbf{curriculum\_threshold}: difficulty is increased whenever the error rate is below this threshold.
 \item \textbf{min\_level\_duration}: minimal number of batches processed between two consecutive increases of the difficulty level.
 \item \textbf{noise\_variance}: \todo{???}
 \item \textbf{noise\_variance\_decay}: the noise variance gets multiplied by this value after every epoch
 \item \textbf{rnn\_size}: the number of LSTM cells and sizes of all hidden layers.
 \item \textbf{reg}: the number of registers.
 \item \textbf{mod\_exec}: the number of times the sequence of standard modules from Sec.~\ref{sec:modules} is repeated
 (See Sec.~\ref{sec:modules} for details).
 \item \textbf{use\_lstm}: LSTM controller is used if this value is set to true.
 \item \textbf{steps}: the number of timesteps in each execution.
 
\end{enumerate}



\subsection{Values of the hyperparameters}\label{app:values}


